Learning Constrained Corner Node Trajectories of a Tether Net System for Space Debris Capture

The earth's orbit is becoming increasingly crowded with debris that poses significant safety risks to the operation of existing and new spacecraft and satellites. The active tether-net system, which consists of a flexible net with maneuverable corner nodes launched from a small autonomous spacecraft, is a promising solution for capturing and disposing of such space debris. The requirement of autonomous operation and the need to generalize over scenarios with debris scenarios in different rotational rates makes the capture process significantly challenging. The space debris could rotate about multiple axes, which, along with sensing/estimation and actuation uncertainties, calls for a robust, generalizable approach to guiding the net launch and flight - one that can guarantee robust capture. This paper proposes a decentralized actuation system combined with reinforcement learning for planning and controlling this tether-net system. In this new system, four microsatellites with cold gas type thrusters act as the corner nodes of the net and can thus help control or correct the flight of the net after launch. The microsatellites pull the net to complete the task of approaching and capturing the space debris. The proposed method uses a RL framework that integrates a proximal policy optimization to find the optimal solution based on the dynamics simulation of the net and the microsatellites performed in Vortex Studio. The RL framework finds the optimal trajectory that is both fuel-efficient and ensures a desired level of capture quality.

==> tables/symsParam_2.tex <==
\caption{\label{tab:table1} Simulation Parameters.}
\centering
% \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccc}
\hline
Parameter&Value\\\hline
\multicolumn{5}{c}{\textbf{Chaser, Tether, and Winch}}\\
\hline
Chaser Side Length $L_{ch}$, m & 1.5\\
Chaser Mass $m_{ch}$, kg & 1600\\
Chaser and Net Initial Distance $d_{ch}$, m & 0.1\\
Winch Radius $r_{w}$, m & 0.05\\
Winch Height $h_{w}$, m & 0.02\\
Winch Mass $m_{w}$, kg& 0.1\\
Tether Radius $r_{t}$, m & 0.002\\
Tether Density $\rho_{t}$, kg/m$^3$& 1390\\
Tether Young's Modulus $E_{t}$, GPA& 70\\
Tether Axial Damping Ratio $c_{t}$& 0.106\\
\hline
\multicolumn{5}{c}{\textbf{Net and Corner Threads}}\\
\hline
Side Length $L_{net}$, m& 22.0\\
Mesh Length $l_{net,0}$, m& 1.0\\
Thread Radius $r_{net}$, m& 0.0011\\
Thread Density $\rho_{net}$, kg/m$^3$& 1390.0\\
Net Young's Modulus $E_{net}$, GPA& 70\\
Net Axial Damping Ratio $c_{net}$& 0.106\\
Corner Thread Length $l_{CT,0}$, m& 1.4142\\
Corner Thread Radius $r_{CT}$, m& 0.0007 \\
\hline
\multicolumn{5}{c}{\textbf{Initial Conditions}}\\
\hline
MU Ejection Speed $v_{e}$, m/s& 2.5\\
MU Shooting Angle $\theta_e$, deg &     36.87 \\
Net Stowed Side Length $L_{net,0}$, m  &     1.1 & \\
\hline
\multicolumn{5}{c}{\textbf{Simulation Setup}}\\
\hline
% Final Time $t_{f}$, s & 120 & Time Step $\Delta$t, s & 10$^{-3}$\\
Time Step $\Delta$t, s & 10$^{-2}$\\
\hline
\label{tab:nominalparams}\\
\end{tabular}
